Representations Before Pixels: Semantics-Guided Hierarchical Video Prediction

Accurate future video prediction requires both high visual fidelity and consistent scene semantics, particularly in complex dynamic environments such as autonomous driving. We present Re2Pix, a hierarchical video prediction framework that decomposes forecasting into two stages: semantic representation prediction and representation-guided visual synthesis. Instead of directly predicting future RGB frames, our approach first forecasts future scene structure in the feature space of a frozen vision foundation model, and then conditions a latent diffusion model on these predicted representations to render photorealistic frames. This decomposition enables the model to focus first on scene dynamics and then on appearance generation. A key challenge arises from the train-test mismatch between ground-truth representations available during training and predicted ones used at inference. To address this, we introduce two conditioning strategies, nested dropout and mixed supervision, that improve robustness to imperfect autoregressive predictions. Experiments on challenging driving benchmarks demonstrate that the proposed semantics-first design significantly improves temporal semantic consistency, perceptual quality, and training efficiency compared to strong diffusion baselines. We provide the implementation code at https://github.com/Sta8is/Re2Pix

==> tables/table_comp_methods.tex <==
\begin{table}
\footnotesize
\centering
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{l cccc cc} \toprule
\mr{2}{\Th{Method}} & \multicolumn{4}{c}{\Th{Perception}} & \multicolumn{2}{c}{\Th{Generation}} \\ 
\cmidrule(lr){2-5} \cmidrule(lr){6-7}
 & mIoU(A)\Th{$\uparrow$} & IoU(M)\Th{$\uparrow$} & $\delta_1$\Th{$\uparrow$} & AbsR\Th{$\downarrow$} & \Th{FID}$\downarrow$ & \Th{FVD}$\downarrow$    \\
\midrule 
Baseline & 60.55 & 57.64 & 85.15 & .1460 & 12.86 & 60.70  \\
w/ REPA \citep{leng2025repa} & 61.45 & 59.63 & 85.35 & .1465& 12.34 & 55.15  \\
w/ VideoREPA \citep{zhang2025videorepa} & 60.98 & 58.61 & 85.22 & .1466 & 12.95 & 59.03 \\
Baseline-Large & 61.69 & 59.65 & 85.43 & .1449 & 11.99 & 56.81 \\
\ours & \textbf{63.53} & \textbf{62.29} & \textbf{85.72} & \textbf{.1413} & \textbf{9.90} & \textbf{52.66} \\ 
\bottomrule
\end{tabular}

\caption{\textbf{Comparison with Baselines.} Our hierarchical method outperforms standard denoising and REPA-based approaches across semantic consistency (perception) and generation metrics. Model parameters: Baseline (782M), REPA methods (792M), Baseline (Large) (1.5B), DINO-FS(258M), \ours (1.1B).}

\label{tab:methods_comparison}
\end{table}

